Automating Formal Verification with Reinforcement Learning and Recursive Inference

Automated formal verification remains challenging for large language models because data for proof assistants and verification-aware languages is scarce, and correctness depends on satisfying precise machine-checkable specifications rather than producing plausible code. This thesis studies how verifier environments can improve LLM generation of verified programs and proofs through reinforcement learning from verifiable rewards (RLVR) and verifier-guided inference-time search. First, we train open-source models in Dafny with RLVR using Group Relative Policy Optimization (GRPO) and related variants, assembling generated candidates into complete programs and scoring them with compiler and verifier outcomes. Initial experiments on an APPS-derived Dafny dataset increased verified reward from 2.2% to 58.1%, but revealed specification hacking, where models exploit weak formal specifications instead of implementing the intended solutions. After filtering underspecified and vulnerable tasks, multi-turn RLVR on the refined benchmark improves the verified pass rate from 9.7% to 31.1%. Second, we develop a verifier-guided inference scaffold in Lean that treats proof generation as structured search over decomposed subgoals, verifier feedback, diagnostics, and repair. With a fixed base model, the full scaffold with proof reviser improves pass rate on an initial VeriCoding pilot set from 46.2% under direct repair to 69.2%. On the larger VERINA dataset, whole-task decomposition plus proof reviser solves 7 of 42 previously unsolved tasks. We also introduce Dalek-Bench, a repository-scale Lean benchmark derived from the Rust $\texttt{curve25519-dalek}$ verification project; preliminary results remain weak, indicating that stronger progress evaluation and task-specific tool-use policies are still needed.

==> fontsets/mitthesis-defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2026/01/31 v1.07 Load Computer/Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Computer Modern text and math fonts (default for pdftex)}
	\RequirePackage[T1]{fontenc} % With T1 encoding, pdftex will silently load the cm-super fontset
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{bm}
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-fira-newtxsf.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-fira-newtxsf.tex}[2026/01/31 v1.07 Load Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font]

%% Adjusted sizes of text, math, and typewriter fonts, 2024/10/11
%% Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Fira sans text font with newtx sans serif math font and Inconsolata typewriter}
	\RequirePackage[U,T1]{fontenc}
    \RequirePackage[varqu,varl]{zi4} % inconsolata font for typewriter
    \RequirePackage[sfdefault,tabular,lf]{FiraSans} % sans serif text package
    % Use option lf to get lining figures rather than default, old style figures. Use tabular to get tabular figures, not proportional figures.
    % Best choice will vary, depending on what type of content you have. With some effort, these settings can be changed according to content,
    % See, e.g.: https://tex.stackexchange.com/q/114331/119566
    \renewcommand\rmdefault{\fira@family} % roman font for math (e.g., for operators) and for \textrm{..}
    \RequirePackage[scaled=1.1]{newtxsf}  % sans serif math; [noSTIXops] option suppresses STIX figures in favor of text font figures, 
    % in the most recent versions of newtxsf, but using the following for backward compatibility. NB: 'figures' means numbers: 0123456789.
    % This matters, for example, in tables that mix text and math figures.
        \DeclareSymbolFont{mynumbers}{T1}{FiraSans-TLF}{m}{n}
        \DeclareMathSymbol{0}{\mathord}{mynumbers}{`0}
        \DeclareMathSymbol{1}{\mathord}{mynumbers}{`1}
        \DeclareMathSymbol{2}{\mathord}{mynumbers}{`2}
        \DeclareMathSymbol{3}{\mathord}{mynumbers}{`3}
        \DeclareMathSymbol{4}{\mathord}{mynumbers}{`4}
        \DeclareMathSymbol{5}{\mathord}{mynumbers}{`5}
        \DeclareMathSymbol{6}{\mathord}{mynumbers}{`6}
        \DeclareMathSymbol{7}{\mathord}{mynumbers}{`7}
        \DeclareMathSymbol{8}{\mathord}{mynumbers}{`8}
        \DeclareMathSymbol{9}{\mathord}{mynumbers}{`9}
 	\RequirePackage{bm}
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassWarning{\ClassName}{The fira-newtxsf font set requires pdflatex. Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-heros-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-heros-stix2.tex}[2025/10/23 v1.08 Load TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font]

%% TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
%
\ifpdftex
	\ClassError{\ClassName}{The heros-stix2 fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=heros-stix2] you must use a unicode engine, such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{TeX Gyre Heros (sans serif) text font with STIX2 math font and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    \setmainfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
    \setsansfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
   \setmonofont{Inconsolatazi4}[
        Scale=1.04,
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02}, % drop +ss03 (upright quotes), 2025/04/18
    ]             
    \setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes helpful
    	Scale=MatchLowercase,%0.95,%MatchUppercase,%MatchLowercase,
		% scaling is a matter of taste ... the x-heights of STIX2 are greater than for Heros...
    	Extension = .otf,
%		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
    ]
    % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
    %    
    \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Heros bold, https://github.com/stipub/stixfonts
    \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
    \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX Two
     %         
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-libertinus.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-libertinus.tex}[2025/09/23 v1.02 Load Libertinus and related fonts]

%% Libertinus (serif) text font with newtxmath[libertinus] (pdftex) or Libertinus (unicode) math font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%  		https://ctan.org/tex-archive/fonts/libertine/opentype 
%		https://github.com/alerque/libertinus
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Libertinus type1 text fonts and newtx-libertinus math fonts}
    \RequirePackage[T1]{fontenc}
    \RequirePackage[lf,t,semibold,ScaleTT=0.9]{libertinus} % tabular lining figures
    \RequirePackage[libertinus,vvarbb,subscriptcorrection]{newtxmath}% see package documentation for options
    \RequirePackage{bm}% load after all math to give access to bold math
\else
	\ClassNoteNoLine{\ClassName}{Loading Libertinus OTF text and math fonts}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode math loads the fontspec package
 	%
    \setmainfont{LibertinusSerif}[% 
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Semibold, 
    	BoldItalicFont = *-SemiboldItalic,
    	RawFeature={+ss05,+dlig,+tnum,+liga}, 
		% +ss02 would change J, K, R; +ss05 changes W; onum = oldstyle figures; hlig = historical ligatures
    ]    
    \setsansfont{LibertinusSans}[% 
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
	    BoldItalicFont = *-Bold,% does not have bold italic
    	Scale=MatchUppercase,
		RawFeature={+liga,},
	]
	%
    \setmonofont{LibertinusMono}[% 
    	Scale=0.9,% 2024/10/13
	    Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Regular,% does not have italic
    	BoldFont = *-Regular,% does not have bold 
	    BoldItalicFont = *-Regular,% does not have bold italic
	] 
	% 
	\newfontfamily\LibertinusDisplay{LibertinusSerifDisplay-Regular.otf}% a display font, as for titles
	%
	\newfontfamily\LibertinusInitials{LibertinusSerifInitials-Regular.otf}% Large initial letters, as for first word in chapter
	%	     	
    %% a Libertinus math font
    \setmathfont{libertinusmath-regular}[%
     	Extension = .otf,   
    	Scale=MatchUppercase,
%		BoldFont = *,% This font lacks a bold version; you could use FakeBold as a stand in
    	RawFeature={+ss08},% +ss08 gives slanted integrals (no other features) 	
    	]
	\setmathfont{Latin Modern Math}[range=\nabla,Scale=0.91] % I hate the backward nabla in Libertinus Math...
	
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-lmodern.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lmodern.tex}[2025/09/23 v1.01 Load Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts}
	\RequirePackage[T1]{fontenc}
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{lmodern}
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-lucida.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lucida.tex}[2026/01/31 v1.06 Load Lucida fonts]

%% Lucida Bright and Lucida Bright Math fonts (available from the TeX Users Group)

\ClassNoteNoLine{\ClassName}{Lucida Bright and Lucida Bright Math fonts}

\ifpdftex
	\RequirePackage[LY1]{fontenc}
	\RequirePackage[expert,vargreek,altbullet]{lucidabr}   % switch text and math fonts 
	% some other options: seriftt (much larger quad size!), lucidasmallscale % 2024/10/13
	\RequirePackage{bm}
\else
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    % FEATURE 	DESCRIPTION 											DEFAULT
    % dlig 		discretionary ligatures (f-ligatures in typewriter fnt) off
    % liga 		standard ligatures (f-ligatures, not monospaced fonts) 	on
    % onum 		old style numbers (Lucida Bright only)					off
    % smcp 		small caps 	(Lucida Bright, upright only)				off
    % zero 		slashed zero (sans and monospaced fonts)				off
    % locl 		script/language specific (localized) forms 				on
    %
    % FEATURE 	FONT 						DESCRIPTION
    % ss01 		Lucida Sans & Typewriter 	use dotted zero: 𝟶 vs. default 0.
    % ss01 		use Lucida-standard shapes:
    % 			Lucida Grande Mono 			ØOQ vs. default 0OQ;
    % 			Lucida Console 				ØOQ vs. default 0OQ.
    
    \setmainfont{LucidaBrightOT}[% main rm
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    %     BoldItalicFeatures={Color=Purple4}, % fixed 2024/10/13
    %     UprightFeatures={Color=Salmon3},
    	  Scale=0.93,% increased from 0.92, 2024/10/13
    %	  Numbers ={OldStyle}, 
      ]
    %
    \setsansfont{LucidaSansOT}[% main sans
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    	  Scale=MatchUppercase,
      ]
    %
    \setmonofont{LucidaSansTypewriterOT}[% main typewriter
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Oblique,
          BoldFont=*-Bold,
          BoldItalicFont=*-BoldOblique,
          Scale=MatchLowercase,% changed from MatchUppercase, 2024/10/13
      ]
    
    %% MATH FONTS
    %
    % ss01 	alternate Latin lower case math italic identical to text italic. This option is not recommended as Greek 𝜈 (nu) and Latin 𝑣 (vee) become too similar
    % ss02 	smaller arrows (original Type 1 size): ⇑ vs. default ⇑.
    % ss03 	attempt to imitate Type 1 fonts
    % ss04 	calligraphic alternative (similar to the Type 1 design) to the math script alphabet
    % ss05 	use a slashed-zero style for the empty set character (U+2205): Ø vs. default ∅
    % ss08 	emphasize right and bottom edges of the d’Alembertian operator (U+29E0, \laplac), to follow the design of the Laplace operator (U+2206, \increment, Δ); the default design emphasizes the left and upper edges. Also available in the bold math font.
    %
    \setmathfont{LucidaBrightMathOT}[% main math
    	  Scale=MatchUppercase,
    	  Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
%    	  BoldFeatures={Color=Chartreuse4},
    	  RawFeature ={+ss04,+ss08}, %
    ]
 
%% LucidaMath-OT contains a *serif* typerwriter font. If you prefer a sans serif typerwriter font, you can use the following two settings. 
% 
%    \setmathfont{LucidaSansTypewriterOT}[% <== NB: setting a text font where math font should go.
%    	  Scale=MatchUppercase,
%          range=tt,
%    	  Color=NavyBlue,
%          Extension=.otf,
%          script-features = {},     
%          sscript-features = {},     
%    	  BoldFont=LucidaSansTypewriterOT-Bold.otf,
%    	  BoldFeatures={Color=Salmon3},
%    ]
%    %
%    \setmathfontface\mathtt{LucidaSansTypewriterOT-Bold}[% bold upright typewriter font in boldmath.
%    	  version=bold,
%    	  Scale=MatchUppercase,
%          Extension=.otf,    
%    ]
	%
    \setmathfont{LucidaBrightMathOT}[%
    	  range={scr},% to make scr differ from cal
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,% could be overridden by bold separate version
    ]
    \setmathfont{LucidaBrightMathOT}[% -Demi .. sufficient this way, since bold set above.
    	  range={bfscr},% need to call \symbfscr manually - bug in unicode-math version & range interaction
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
    ]
    %% Fix unicode-math operator font not set up for bold face (default \mathrm). See https://github.com/wspr/unicode-math/issues/468
    \setoperatorfont\symup
    %
    % note \mathbfit = \symbfit
    
    % The specialized one-off Lucida fonts:
    \newfontface\LucidaBlackletter{LucidaBlackletterOT}[%
    	Scale=0.95,% <== NB
    	Extension=.otf,
    	]
    \newfontface\LucidaCalligraphy{LucidaCalligraphyOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
    	]
    \newfontface\LucidaHandwriting{LucidaHandwritingOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
     	]
    % GrandeMono and Console fonts:
    \newfontface\LucidaGrandeMonoDK{LucidaGrandeMonoDK}[%	
    	Scale=MatchUppercase,
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
    \newfontface\LucidaConsole{LucidaConsoleDK}[%
    	Scale=MatchLowercase,% <=== NB
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
\fi
%
\RequirePackage{etoolbox} % may already be loaded by the .cls file
% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}


==> fontsets/mitthesis-newtx-sans-text.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx-sans-text.tex}[2026/01/31 v1.05 Load newtx sans-serif text and regular math fonts]

%% newtx package with sans-serif text (Helvetica-like text with Times-like math)
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading newtx sans-serif text and newtx serif math fonts}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91,defaultsups]{newtx}% upint for upright integrals
	\AtEndPreamble{% added to accommodate v1.731 of newtx, 2023/11/03
	    \renewcommand{\familydefault}{\sfdefault}% use sans for main text
%	    \renewcommand{\rmdefault}{\sfdefault}% uses sans for \textrm{}, if that's desired.
	}
%   these two commands enable hyphenation of the typewriter font - https://tex.stackexchange.com/a/204421/119566
%    \input{t1ntxtt.fd}
%    \DeclareFontFamily{\encodingdefault}{\ttdefault}{\hyphenchar\font=`\-} % 
	\RequirePackage{bm}% bold math
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassWarning{\ClassName}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-newtx.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx.tex}[2026/01/31 v1.05 Load newtx text and math fonts]

\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading newtx fonts with inconsolata typewriter}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91]{newtx}% stix2, upint
    \RequirePackage[varl,varqu,hyphenate,mono]{inconsolata}% sans typewriter font; mono = fixed word spacing, hyphenate = allow hyphenation 
	\RequirePackage{bm}
	\let\textsuperscript\textsu% newtx changes the default superiors font; this is needed to get commas aligned in sequential footnotes
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassWarning{\ClassName}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-stix2.tex}[2025/09/23 v1.08 Load STIX Two text and math fonts]

%% STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%				https://github.com/stipub/stixfonts 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://ctan.org/tex-archive/fonts/inconsolata
%
\ifpdftex
	\ClassError{\ClassName}{The stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}{Use LuaLatex to run with the class option [fontset=stix2]}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{STIXTwoText}[
       	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
	]
	\setsansfont{texgyreheros}[ 
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% 
	]        
	\setmonofont{Inconsolatazi4}[
        Scale=1.035,% 2024/10/13
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02}, % drop +ss03 (upright quotes), 2025/04/18
    ]             
	\setmathfont{STIXTwoMath-Regular}[
    	Scale=MatchUppercase,
    	Extension = .otf,
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes-stix2.tex}[2025/09/23 v1.08 Load TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font]

%% TeX Gyre Termes text font and Heros sans serif font with STIX2 math font and Inconsolata monospaced font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
%
\ifpdftex
	\ClassError{\ClassName}{The termes-stix2 fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=termes-stix2], use a unicode engine such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[
		WordSpace = {1,1.4,1},%% This stretch matches newtxtext a little better. 1.4
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
	\setsansfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]        
	\setmonofont{Inconsolatazi4}[
        Scale=1,% reset to 1, 2024/10/12 %1.03,% rescaled from 1, 22/03/10
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02}, % drop +ss03 (upright quotes), 2025/04/18
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes helpful
    	Scale=MatchUppercase,
    	Extension = .otf,
%		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Termes bold
   \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
   \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX, not Termes
    %      
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes.tex}[2025/09/23 v1.07 Load TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font]

%% TeX Gyre Termes (Times-like) text font with Termes math font and Heros sans serif font and Cursor monospaced font
%
%  These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%  They are also available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
%
\ifpdftex
	\ClassError{\ClassName}{The termes fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=termes], use a unicode engine such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[
		WordSpace = {1,1.4,1},
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
    \setsansfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as used in newtx; former value 0.9 too small 2022/01/15
	]        
   \setmonofont{texgyrecursor}[
        %Scale=0.97,
        Scale=1.03, % adjusted 2024/10/12 to bring x-size closer to other fonts
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Italic,
        BoldFont = *-Bold, 
    	BoldItalicFont = *-BoldItalic,
%		BoldFeatures = { Color = VioletRed3 },
    ]             
    \setmathfont{texgyretermes-math}[
    	Scale=MatchUppercase,
    	Extension = .otf,
%		BoldFont = *, % termes-math does not have a bold version
%       Color=Red3, 
    ]
    %   
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}
\fi

